Studying Logging Practice in Machine Learning-based Applications

Logging is a common practice in traditional software development. Several research works have been done to investigate the different characteristics of logging practices in traditional software systems (e.g., Android applications, JAVA applications, C/C++ applications). Nowadays, we are witnessing more and more development of Machine Learning-based applications (ML-based applications). Today, there are many popular libraries that facilitate and contribute to the development of such applications, among which we can mention: Pytorch, Tensorflow, Theano, MXNet, Scikit-Learn, Caffe, and Keras. Despite the popularity of ML, we don't have a clear understanding of logging practices in ML applications. In this paper, we aim to fill this knowledge gap and help ML practitioners understand the characteristics of logging in ML-based applications. In particular, we conduct an empirical study on 110 open-source ML-based applications. Through a quantitative analysis, we find that logging practice in ML-based applications is less pervasive than in traditional applications including Android, JAVA, and C/C++ applications. Furthermore, the majority of logging statements in ML-based applications are in info and warn levels, compared to traditional applications where info is the majority of logging statement in C/C++ application and debug, error levels constitute the majority of logging statement in Android application. We also perform a quantitative and qualitative analysis of a random sample of logging statements to understand where ML developers put most of logging statements and examine why and how they are using logging. These analyses led to the following observations: (i) ML developers put most of the logging statements in model training, and in non-ML components. (ii) Data and model management appear to be the main reason behind the introduction of logging statements in ML-based applications.

==> declaration.tex <==
% Declarations

% Funding 
% No funding was received for conducting this study.

% Conflicts of interest/Competing interests
% The authors have no relevant financial or non-financial interests to disclose.

% Availability of data and material
% The datasets generated during and/or analysed during the current study are available in the Github repository, https://github.com/senseconcordia/TestLoggingPractice.

% Code availability
% Code for data cleaning and analysis is provided as part of the replication package. It is available at https://github.com/senseconcordia/TestLoggingPractice.

% \begin{titlepage}
%     Declarations

% Funding 
% No funding was received for conducting this study.

% Conflicts of interest/Competing interests
% The authors have no relevant financial or non-financial interests to disclose.

% Availability of data and material
% The datasets generated during and/or analysed during the current study are available in the Github repository, https://github.com/senseconcordia/TestLoggingPractice.

% Code availability
% Code for data cleaning and analysis is provided as part of the replication package. It is available at https://github.com/senseconcordia/TestLoggingPractice.
% \end{titlepage}

==> rq4.tex <==
\subsection*{\textbf{RQ4:} What is the relationship between test logging and production logging?}

\subsubsection*{Motivation}

During the software testing process, both production and test logs are printed. A production log displays production information under testing while a test log is generated by a test suite.  RQ1 and RQ2 highlight some significant differences and similarities in logging practices between test and production files, implying that test logs may not be independent of production logs. In this case, the question arises as to whether the log information contained in test logs could be useful for production logging, for example, to leverage the information in test logs to improve production logging statements. Therefore, to answer this question, we conduct a manual study to explore the relationships between test and production logging. Based on the results of the manual study, we classify the test logs to determine whether the information in the test log is useful for production logging. We would like to know, even though test logs are generated by test files, if they are added to production logging, whether they can help people better understand the runtime behavior of the system.
To the best of our knowledge, this is the first study to investigate the relationship between test logging and production logging and classify test logs' usefulness for production logging.

\subsubsection*{Approach}
As shown in \autoref{fig:rq4workflow}, our approach consists of three steps. In the first step, we execute all of the unit tests for the subjects under investigation in order to obtain test outputs\footnote{In this work, we refer to test outputs as the log messages produced during the execution of the unit tests.}. The second step takes the test outputs from the first step as input and uses regular expressions to identify the test logs from them. In the final step, we randomly select a sample from the test logs identified in the previous step and label each test log using a pair review. These labels reflect the relationship between test logs and their corresponding production logs, as well as whether the information supplied by the test logs is useful for production logging and the test log's classification.

\begin{figure}[htp]
    \includegraphics[scale=0.25]{rq4_research_workflow.png}
    \centering
    \caption{Overview of the research approach for RQ4.} 
    \label{fig:rq4workflow} 
\end{figure}

\begin{itemize}
\item \textbf{Tests outputs collection.} 
We begin by cloning the research subjects onto our local machine.
Because all of the research subjects use automation build tools, such as \ji{maven} and \ji{ant}, for software building and testing that publishes logs through \textit{Terminal}, we modify the test configuration files to redirect the test outputs from \textit{Terminal} into text files to facilitate further data analysis. Finally, we execute the tests through the command line. For example, we run all the tests of the subjects that use \ji{maven} as their automation build tool with \ji{mvn clean install -fn}.

\item \textbf{Log messages identification.} 
Each text file generated in the first step contains test logs and production logs produced by the production code covered by the test case involved in this text file. The goal of this step is to identify test logs so that we can investigate the relationships between them and the other logs (i.e., production logs) in the following step.
A typical test log would appear like this:

\vspace{0.2cm}
\wrapcolorbox[gray!10]{2021-01-27 17:19:13,973 INFO  [pool-1-thread-4] amrmproxy.TestAMRMProxyService (TestAMRMProxyService.java:invoke(402)) - Sucessfully registered application master with appId: 3} 

We first use regular expressions to match the time patterns to identify the typical logs  (atypical logs are worthless for subsequent analysis), and then we use regular expressions and the search-keyword ``test'' to identify test logs in the test outputs. Typical logs can specify which files generate the logs. In the example above, this log is generated by \ji{TestAMRMProxyService.java}. The keyword ``test'' is always present in the name of a test file so that we can use it to identify test logs. This approach has been proved to have a high precision and an acceptable recall in identifying test and production files~\citep{test_code_traceability}.

\item \textbf{Log messages analysis.} 
In this step, we manually analyze the log information from test and production logs. The reason we adopt the manual analysis method instead of checking the function calls is that checking function calls is a coarse-grained approach. The presence of a production method invocation in a test does not imply that the test logs generated by this test can be helpful to the production logging. Finding the relationships between test and production logging requires the analysis of log information, and human effort is needed to understand log information. We first sample the test logs and then apply two rounds of labeling to the logs samples. We randomly sample test logs with five confidence interval and 95\% confidence level \citep{sample_size_calculator}. We obtained 385 different test log samples from the unit tests' outputs that contain 691,310 instances in total, and selected 100 logs at random from this log sample set to perform the first round of labeling. Our log samples are divided into five batches, each of which is reviewed by two researchers individually, due to the fact that there are five researchers involved in this study. Each test log is provided with the context of the test output which includes all the production and test logs produced during the execution of a unit test. 


The first round of labeling only examines a subset of the log samples in order to obtain an initial consensus and get some common knowledge. The first round of labeling produces a preliminary set of labels used for the second round. The labeling is based on  log content analysis of test logs and the surrounding production logs in the same log file, which necessitates that the labelers comprehend the log information in test logs and the surrounding production logs. The second round of labeling covers all log samples and is based on the common understanding of the prior round. The second round includes labeling the rest of the test logs as well as revisiting the labeled logs to alter them if they are against the established knowledge base. If the two researchers are unable to achieve an agreement, a third researcher may be invited to reach the final agreement. 
After these two rounds of labeling, the \textit{Cohen's kappa} of researcher agreement ranges from 0.91 to 1 for three labels, indicating that researchers attain a consistent agreement on the test log labels. The final agreement was then reached with the assistance of a third researcher.

\end{itemize}

\subsubsection*{Results}
Each test log sample has three labels: (1) the relationships between it and the relevant surrounding production logs, (2) the usefulness of test logs for production, and (3) test log classifications. Below are the details of these three labels:

\paragraph{\textbf{\textup{Relationship between the test logs and production logs.}}} As shown in \autoref{fig:relationship_pie_chart}, our research has yielded four categories with regard to the relationship between test and production logs: \textit{Test only}, \textit{Overlap}, \textit{Elaboration}, and \textit{Complementary}. The definition of each category is provided below, along with an example in table \autoref{tab:test_production_relationship}. The fonts of labeled test logs are in `blue color', while the fonts of associated production logs are in `orange color'. In every category, we display not only the labeled test logs but also logs that surround them to help readers understand the context of each test log.

\begin{table}[htp]
\footnotesize
\caption{Relationships between test and production logs.}
\label{tab:test_production_relationship}
\centering
\begin{tabular}{|m{0.17\textwidth}|m{0.76\textwidth}|}
\hline
\textbf{Relationship}
& \textbf{Example}\\
\hline
Test only
&
\vspace{0.1cm}

\wrapcolorbox[gray!10]{
2021-03-01 22:23:45,738 INFO  [Time-limited test] wal.AbstractFSWAL(990): Closed WAL: AsyncFSWAL hregion-45030200:(num 1614655425101)

{\color{dodgerblue}
2021-03-01 22:23:45,738 INFO  [Time-limited test] hfile.TestScannerFromBucket
Cache(94): Cleaning test directory:/anonymous/hbase-master/hbase-server/target/
test-data/anonymous
}

2021-03-01 22:23:45,755 INFO  [Time-limited test] hbase.ResourceChecker(179): after: io.hfile.TestScannerFromBucketCache\#testBasicScanWithOffheapBucketCache
WithMBB Thread=39 (was 26) - Thread LEAK? -, OpenFileDescriptor=358 (was 310) - OpenFileDescriptor LEAK? -, MaxFileDescriptor=1048576 (was 1048576), SystemLoadAverage=77 (was 77), ProcessCount=122 (was 122), AvailableMemoryMB=1831 (was 2244)
}



\textsl{(a) Generated by TestScannerFromBucketCache (subject: \hbase)}
\\
\hline
Overlap
&
\vspace{0.1cm}
\wrapcolorbox[gray!10]{
{\color{orange}
2020-12-10 17:39:27,707 [main           ] - INFO  KahaDBDeleteLockTest           - Lock file /anonymous/activemq-master/activemq-unit-tests/target/activemq-data/KahaDBDeleteLockTest/kahadb/lock, last mod at: Thu Dec 10 17:39:27 EST 2020}

{\color{dodgerblue}
2020-12-10 17:39:30,078 [KeepAlive Timer] - INFO  LockFile                       - Lock file /anonymous/activemq-master/activemq-unit-tests/target/activemq-data/KahaDBDeleteLockTest/kahadb/lock, locked at Thu Dec 10 17:39:27 EST 2020, has been modified at Thu Dec 10 17:39:29 EST 2020}
}
\textsl{(b) Generated by KahaDBDeleteLockTest (subject: \actvieMQ)}
\\
\hline
Elaboration
&
\vspace{0.1cm}

\wrapcolorbox[gray!10]{

{\color{orange}
2021-01-27 17:17:17,627 INFO  [main] scheduler.DistributedOpportunisticContainerA-
llocator (DistributedOpportunisticContainerAllocator.java:allocateContainersIntern-
al(227)) - Opportunistic container has already been allocated on h3.}

{\color{dodgerblue}
2021-01-27 17:17:17,627 INFO  [main] scheduler.TestDistributedOpportunisticConta-
inerAllocator (TestDistributedOpportunisticContainerAllocator.java:testMaxAlloca-
tionsPerAMHeartbeat(669)) - Containers: [Container: [ContainerId: container\_0\_0-
001\_01\_000002, AllocationRequestId: -1, Version: 0, NodeId: h3:1234, NodeHttpAd-
dress: h3:1234, Resource: <memory:1024, vCores:1>, Priority: 1, Token: Token { kind: ContainerToken, service: h3:1234 }, ExecutionType: OPPORTUNISTIC, ], Container: [ContainerId: container\_0\_0001\_01\_000003, AllocationRequestId: -1, Version: 0, NodeId: h2:1234, NodeHttpAddress: h2:1234, Resource: <memory:1024, vCores:1>, Priority: 1, Token: Token { kind: ContainerToken, service: h2:1234 }, ExecutionType: OPPORTUNISTIC, ]]}

}

\textsl{(c) Generated by TestDistributedOpportunisticContainerAllocator (subject: \hadoop)}
\\
\hline
Complementary
&
\vspace{0.1cm}

\wrapcolorbox[gray!10]{
{\color{orange}
2021-01-27 17:37:04,213 INFO  [Container Monitor] monitor.ContainersMonitorImpl (ContainersMonitorImpl.java:run(512)) - Skipping monitoring container container\_123456\_0001\_01\_000001 since CPU usage is not yet available.}

{\color{dodgerblue}
2021-01-27 17:37:04,233 INFO  [main] monitor.TestContainersMonitorResourceChange (TestContainersMonitorResourceChange.java:waitForContainerResourceUtilizationC-
hange(326)) - Monitor thread is waiting for resource utlization change.}

{\color{orange}
2021-01-27 17:37:04,254 WARN [Container Monitor] monitor.Container-
sMonitorImpl (ContainersMonitorImpl.java:run(561)) - org.apache.hadoop.yarn-
.server.nodemanager.containermanager.monitor.ContainersMonitorImpl is interrupted. Exiting.}
}
\textsl{(d) Generated by TestContainersMonitorResourceChange  (subject: \hadoop)}
\\
\hline
\end{tabular}
\end{table}

\begin{itemize}
\item \textbf{Test only (290/385).} Test logs in this category only contain information about the tests and do not include any relevant production logs in the same file. As illustrated in \autoref{tab:test_production_relationship}, the test log refers to cleaning up a directory used for testing only during a test.

\item \textbf{Overlap (40/385).} 
In this category, the information provided by test logs is also reflected in production logs. For example, the test log (`blue' font) and related production log (`orange' font) in \autoref{tab:test_production_relationship} are both indicating the same file is locked therefore this test log is overlapping with production logs.

\item \textbf{Elaboration (29/385).} 
Test logs in this category contain information that somewhat overlaps with relevant production logs, but they elaborate the production logs with additional details. In \autoref{tab:test_production_relationship}, although the production log includes information about the \ji{opportunistic container}, the test log provides more details about the \ji{opportunistic container}, such as container ID and version.

\item \textbf{Complementary (26/385).} 
Test logs in this category complement the information conveyed in the production logs. As shown in \autoref{tab:test_production_relationship}, the test log indicates that the monitoring thread is waiting for the required resource to be utilizable while the first production log indicates that CPU usage is not yet available.
\end{itemize}

\begin{figure}[htp]
    \includegraphics[scale=0.45]{rq4_relationship_pie_chart.png}
    \centering
    \caption{Relationship between test and production logs.} 
    \label{fig:relationship_pie_chart} 
\end{figure}

\autoref{fig:relationship_pie_chart} presents proportions for each category of the relationship between production logs and test logs. Based on this figure, the most prevalent relationship is \textit{Test only} (75.3\%). This number confirms developers' intuition that the vast majority of test logs are dedicated to testing rather than production. However, there is quite a large number (around a quarter) of test logs related to production. The second most prevalent relationship is the \textit{Overlap} relationship (10.4\%), which signifies that either the test code developers are not aware of the similar logging in production code, or the production logging is not in a good format that facilitates testing. The least common relationships between test logs and production logs are \textit{Elaboration} (6.8\%) and \textit{Complementary} (7.5\%), both of which have fairly comparable proportion numbers. 

The \textit{Elaboration} and \textit{Complementary} relationships suggest that the production run-time information contained in the production logging is not sufficient for understanding the testing results. Test logs that are labeled with \textit{Overlap} relationship with production logging provide the same information as in production logs, hence we conjecture that such test logs may not be useful to production logging. However, there is no existing evidence (to the best of our knowledge) proving this. Thus, we also examine whether such test logging could be useful and added to the production code. 

\paragraph{\textbf{\textup{Usefulness of test logs.}}}
In the subsequent analysis, we examined the usefulness (to production logging) of the 95 test logs that are not labeled with \textit{Test only} and assigned these logs three labels: \textit{Useful}, \textit{Not useful}, and \textit{Unclear}. Generally, we manually examine the contents of test logs and the production logs that surround them. We would like to know, if the information contained in the test logs is added to production logging statements, whether it can improve production logging and help people better understand the runtime behavior of the system (i.e., being useful). \autoref{tab:test_log_usefulness} presents some examples of useful and useless test logs. As in the previous section, the analyzed test logs are denoted by `blue' font color. \autoref{fig:usefulness_bar_chart} depicts the connections between the usefulness of test logs and their relationship with production logs.

\begin{table}[htp]
\footnotesize
\caption{Example of the usefulness of the test logs.}
\label{tab:test_log_usefulness}
\centering
\begin{tabular}{|m{0.17\textwidth}|m{0.76\textwidth}|}
\hline
\textbf{Usefulness}
& \textbf{Example}\\
\hline
Useful
&
\vspace{0.1cm}
\wrapcolorbox[gray!10]{
2021-01-27 19:43:18,394 INFO  [Thread-179] webapp.RouterWebServices (RouterWebServices.java:initializePipeline(267)) - Initializing request processing pipeline for user: test1

{\color{dodgerblue}
2021-01-27 19:43:18,395 INFO  [Thread-180] webapp.TestRouterWebServices (TestRouterWebServices.java:run(309)) - init web interceptor success for usertest1}
}
\textsl{(a) Generated by TestRouterWebServices (subject: \hadoop)}
\\
\hline
Not useful
&
\vspace{0.1cm}

\wrapcolorbox[gray!10]{
2021-01-27 17:55:54,353 INFO  [main] distributed.CentralizedOpportunistic-
ContainerAllocator (CentralizedOpportunisticContainerAllocator.java:allocatePerSchedulerKey(167)) - Opportunistic allocation requested for [priority=1, allocationRequestId=2, num\_containers=2, capability=<memory:1024, vCores:1>] allocated = [<memory:1024, vCores:1>]

{\color{dodgerblue}
2021-01-27 17:55:54,353 INFO  [main] distributed.TestCentralizedOpportunistic-
ContainerAllocator (TestCentralizedOpportunisticContainerAllocator.java:testAllocationLatencyMetrics(598)) - Containers: [Container: [ContainerId: container\_0\_0001\_01\_000002, AllocationRequestId: 2, Version: 0, NodeId: h1:1234, NodeHttpAddress: null, Resource: <memory:1024, vCores:1>, Priority: 1, Token: Token { kind: ContainerToken, service: h1:1234 }, ExecutionType: OPPORTUNISTIC, ], Container: [ContainerId: container\_0\_0001\_01\_000003, AllocationRequestId: 2, Version: 0, NodeId: h1:1234, NodeHttpAddress: null, Resource: <memory:1024, vCores:1>, Priority: 1, Token: Token { kind: ContainerToken, service: h1:1234 }, ExecutionType: OPPORTUNISTIC, ]]}
}
\textsl{(c) Generated by TestCentralizedOpportunisticContainerAllocator (subject: \hadoop)}
\\
\hline
\end{tabular}
\end{table}

\begin{itemize}
\item \textbf{Useful (35/95).} The information provided by test logs in this category is useful to production logging. As the example shows in \autoref{tab:test_log_usefulness}, the surrounding log is describing the initialization of a requested resource from a specific user, and the target test log is indicating the success of initialization.
\item \textbf{Not useful (57/95).} The information contained in test logs is useless to production logging. For example, the surrounding log in \autoref{tab:test_log_usefulness} describes the properties of an \ji{opportunistic container}. Although the analyzed test log contains more details about this container, it is useless for production logging since this container is primarily used for testing, and details about it are not required in production.
\item \textbf{Unclear (3/95).} Finally, we have observed several test logs that are difficult to determine whether they are useful to production logging due to the lack of related domain knowledge.
\end{itemize}

\begin{figure}[htp]
    \includegraphics[scale=0.45]{rq4_usefulness_bar_chart.png}
    \centering
    \caption{Usefulness of non-\textit{Test-Only} logs.} 
    \label{fig:usefulness_bar_chart} 
\end{figure}

\autoref{fig:usefulness_bar_chart} demonstrates the correlations between the usefulness of test logs and their relationships with production logs. We find that the category \textit{Useful} consists of 20 cases of \textit{Complementary} and 15 cases of \textit{Elaboration}, with no \textit{Overlap}. The category \textit{Not useful} is composed of 6 cases of \textit{Complementary}, 12 cases of \textit{Elaboration}, and 39 cases of \textit{Overlapping}. The majority of \textit{Overlap} cases fall into the category of \textit{Not useful}, which implies the test logs having an \textit{Overlap} relationship with production logging are almost useless to production logging which is because such information is already available in the production logging.


\paragraph{\textbf{\textup{Classification of test logs.}}} 
To further investigate what information makes test logs useful, we then classify the information recorded in the 95 test logs that are not labeled with \textit{Test only} during our subsequent analysis. Our study has revealed ten categories based on the information contained within these logs which can be leveraged in future research with regard to how to identify and utilize the useful information in test logs. These ten categories are defined below, and examples are included in \autoref{tab:test_log_category}. Just as in the previous section, the analyzed test logs are marked with a blue color.

\begin{table}[htp]
\footnotesize
\caption{Classifications of test logs.}
\label{tab:test_log_category}
\centering
\begin{tabular}{|m{0.17\textwidth}|m{0.76\textwidth}|}
\hline
\textbf{Classification}
& \textbf{Example}\\
\hline
\shortstack{Production\\intermediate\\data}
&
\vspace{0.1cm}
\wrapcolorbox[gray!10]{
2021-01-27 20:38:31,249 INFO  [AsyncDispatcher event handler] impl.JobImpl (JobImpl.java:handle(1022)) - job\_0\_0000Job Transitioned from SETUP to RUNNING

{\color{dodgerblue}
2021-01-27 20:38:31,253 INFO  [Listener at 0.0.0.0/46761] hs.TestJobHistoryEvents (TestJobHistoryEvents.java:testHistoryEvents(61)) - JOBID is job\_0\_0000}

}
\textsl{(a) Generated by TestJobHistoryEvents (subject: \hadoop)}
\\
\hline
\shortstack{Test\\intermediate\\data}
&
\vspace{0.1cm}
\wrapcolorbox[gray!10]{
2021-01-27T12:25:02,674  WARN [main] ql.TestTxnNoBuckets: after compact

{\color{dodgerblue}
2021-01-27T12:25:02,674  WARN [main] ql.TestTxnNoBuckets: \{"writeid":
0,"bucketid":536870912,"rowid":4\}	1	4	file:/anonymous/hive-master/ql/target/tmp/org.apache.hadoop.hive.ql.TestTxnNoBuckets-1611779017548/warehouse/nonacidnonbucket/base\_10000004\_v0000023/bucket\_00000}


2021-01-27T12:25:02,674  WARN [main] ql.TestTxnNoBuckets: \{"writeid":
0,"bucketid":536870912,"rowid":5\}	1	5	file:/anonymous/hive-master/ql/target/tmp/org.apache.hadoop.hive.ql.TestTxnNoBuckets-1611779017548/warehouse/nonacidnonbucket/base\_10000004\_v0000023/bucket\_00000}
\textsl{(b) Generated by TestTxnNoBuckets (subject: \hive)}
\\
\hline
\shortstack{Production\\event}
&
\vspace{0.1cm}

\wrapcolorbox[gray!10]{
{\color{dodgerblue}
2021-01-27 17:19:13,973 INFO  [pool-1-thread-4] amrmproxy.TestAMRMProxyService (TestAMRMProxyService.java:invoke(402)) - Sucessfully registered application master with appId: 3}

2021-01-27 17:19:13,974 INFO  [pool-1-thread-1] amrmproxy.BaseAMRMProxyTest (BaseAMRMProxyTest.java:call(251)) - Successfully sent request for context: 0}
\textsl{(c) Generated by TestAMRMProxyService (subject: \hadoop)}
\\
\hline
Test event
&
\vspace{0.1cm}
\wrapcolorbox[gray!10]{
{\color{dodgerblue}
Mar 03, 2021 12:48:26 AM org.apache.tomcat.websocket.server.TestClose\$TestEndpo-
int onOpen INFO: Session opened}

Mar 03, 2021 12:48:26 AM org.apache.tomcat.websocket.server.TestClose\$TestEndpo-
int onMessage INFO: Message received: Test}
\textsl{(d) Generated by TestClose  (subject: \tomcat)}
\\
\hline
\shortstack{Production\\method call}
&
\vspace{0.1cm}
\wrapcolorbox[gray!10]{
{\color{dodgerblue}
2020-12-10 16:12:03,380 [main           ] - INFO  AMQ4636Test                    - *** createDurableConsumer() called ...}

2020-12-10 16:12:03,383 [ActiveMQ Task-1] - INFO  FailoverTransport              - Successfully connected to tcp://anonymous:36205}
\textsl{(e) Generated by AMQ4636Test.java  (subject: \actvieMQ)}
\\
\hline
Test setup
&
\vspace{0.1cm}
\wrapcolorbox[gray!10]{
{\color{dodgerblue}
2021-01-27 12:46:11,576 [Listener at localhost/10990] INFO  ha.TestFailureToReadEdits (TestFailureToReadEdits.java:setUpCluster(130)) - Set SHARED\_DIR\_HA cluster's basePort to 13512}

2021-01-27 12:46:11,576 [Listener at localhost/10990] INFO  hdfs.MiniDFSCluster (MiniDFSCluster.java:<init>(509)) - starting cluster: numNameNodes=2, numDataNodes=0}
\textsl{(f) Generated by TestFailureToReadEdits  (subject: \hadoop)}
\\
\hline
\shortstack{Production\\return}
&
\vspace{0.1cm}
\wrapcolorbox[gray!10]{
2021-01-27 16:40:18,119 [Time-limited test] DEBUG net.NetworkTopology (NetworkTopology.java:chooseRandom(539)) - chooseRandom returning 2.2.2.2:9866

2021-01-27 16:40:18,119 [Time-limited test] DEBUG net.NetworkTopology (NetworkTopology.java:chooseRandom(539)) - chooseRandom returning 9.9.9.9:9866

{\color{dodgerblue}
2021-01-27 16:40:18,119 [Time-limited test] INFO  net.TestNetworkTopology (TestNetworkTopology.java:pickNodesAtRandom(406)) - Result:\{2.2.2.2:9866=4, 20.20.20.20:9866=3, 4.4.4.4:9866=3, 15.15.15.15:9866=7, 17.17.17.17:9866=6, 19.19.19.19:9866=8, 16.16.16.16:9866=9, 9.9.9.9:9866=4, 8.8.8.8:9866=9, 14.14.14.14:9866=2, 7.7.7.7:9866=5, 5.5.5.5:9866=4, 6.6.6.6:9866=5, 12.12.12.12:9866=9, 11.11.11.11:9866=4, 10.10.10.10:9866=5, 18.18.18.18:9866=2, 3.3.3.3:9866=3, 1.1.1.1:9866=0, 13.13.13.13:9866=8\}}}
\textsl{(g) Generated by TestNetworkTopology  (subject: \hadoop)}
\\
\hline
\shortstack{Environmental\\information}
&
\vspace{0.1cm}
\wrapcolorbox[gray!10]{
{\color{dodgerblue}
2021-03-02 00:36:13,370 [myid:] - INFO  [main:ClientPortBindTest@79] - Using [0:0:0:0:0:0:0:1\%lo]:30073 as the host/port}}
\textsl{(h) Generated by ClientPortBindTest  (subject: \zookeeper)}
\\
\hline
Test assertion
&
\vspace{0.1cm}
\wrapcolorbox[gray!10]{
{\color{dodgerblue}
2021-01-27 11:36:35,377 [Listener at localhost/35513] INFO  blockmanagement.TestNameNodePrunesMissingStorages (TestNameNodePrunesMissingStorages.java:get(361)) - Expected blk\_1073741825 to be in storage id DS-2ab551a0-7f03-4b60-8102-ea222efeecbd, but it was in DS-6ab27eb6-9c23-4c21-89bc-cdca79ea996e.  Continuing to wait.}}
\textsl{(i) Generated by TestNameNodePrunesMissingStorages  (subject: \hadoop)}
\\
\hline
\end{tabular}
\end{table}

\begin{itemize}
\item \textbf{Production intermediate data (31/95).} 
In this category, test logs contain information regarding the properties of the software or production code that is being tested. For example, the test log in \autoref{tab:test_log_category} depicts the ID of an ongoing production event.

\item \textbf{Test intermediate data (6/95).} 
Test logs in this category display the intermediate status of the resource exclusively for testing or the temporary values of variables in test code during test execution. In \autoref{tab:test_log_category}, the test log is recording the temporary status of the resources only for testing.

\item \textbf{Production event (21/95).} Test logs in this category depict the events related to the production code under test. The example presented in \autoref{tab:test_log_category} is describing an event about the production code under test.

\item \textbf{Test event (15/95).} 
Test logs in this category portray events that only pertain to the tests rather than the tested production code. The example in \autoref{tab:test_log_category} displays the event of initiating a session, which is exclusively relevant to the test.

\item \textbf{Production method call (1/95).} 
Test logs describe the method invocations in production files for this category. An example in \autoref{tab:test_log_category} obviously mentions a production method \ji{createDurableConsumer()} is invoked.

\item \textbf{Test setup (4/95).} In this category, test logs describe the configuration to set up tests. 
The test log in \autoref{tab:test_log_category} describes how to set up the cluster's (\ji{SHARED_DIR_HA}) port number for testing.

\item \textbf{Production return (5/95).} Test logs in this category record the information returned from the production code. As the example shown in \autoref{tab:test_log_category}, the test log is displaying the node selection result for a network topology which is the return result from production code regarding node selection strategy.

\item \textbf{Environmental information (7/95).}
Test logs in this category display the environmental information of the platform, host, or hardware that the test is running on.

\item \textbf{Test assertion (2/95).} 
In this category, test logs record the assertion results, and always include both expected and actual test results. The example in \autoref{tab:test_log_category} represents the two types of test results in a single log.

\item \textbf{Others (3/95).} In this category, we include those cases not covered by any of the preceding categories.

\end{itemize}

\begin{figure}[htp]
    \includegraphics[scale=0.45]{rq4_category_pie_chart.png}
    \centering
    \caption{Test log categories.} 
    \label{fig:category_pie_chart} 
\end{figure}


\autoref{fig:category_pie_chart} demonstrates the proportion of each category for the test logs not labeled with \textit{Test only}. As it shows in this figure, the most common category is \textit{Production intermediate data} (32.6\%), which indicates that the majority of test logs are leveraged to record the intermediate status of the software or resources under test. The second and the third most common categories are \textit{Production Event} (22.1\%) and \textit{Test Event} (15.8\%) respectively, implying that test logs are often utilized to record the events of production or tests. The least common category is \textit{Production Method Call} (1.1\%). 


